On the Latency of IEEE 802.11ax WLANs with Parameterized Spatial Reuse

In this article, we evaluate the performance of the parameterized spatial reuse (PSR) framework of IEEE 802.11ax, mainly focusing on its impact on transmission latency. Based on detailed standard-compliant system-level simulations, we provide a realistic analysis of the effects of PSR considering different scenario densities, traffic loads, and access points (APs) antenna capabilities to quantify its performance gains under various scenarios. Our results show that, in medium-density scenarios, PSR can offer up to a 3.8x reduction in the 5% worst-case latencies for delay-sensitive stations with respect to an 802.11ax system without PSR. Moreover, our study demonstrates that, for low-latency communications, providing the network with PSR capabilities may be an appealing alternative to the deployment of more costly multi-antenna APs.

==> Section6.tex <==
\section{Conclusions}
\label{sec:conclusions}

We show on our results that, for the simulated deployment, PSR can offer up to $\approx 3.8\times$ smaller worst-case latencies w.r.t the baseline 802.11ax on medium-density scenarios, as well as reducing the $15\%$ worst-case latencies by a factor of $\approx3.8\times$ when the offered traffic load reaches 100Mbps. We also show that, for the short-packet low-latency applications evaluated, even single-antenna APs with PSR capabilities may outperform baseline 802.11ax multi-antenna APs, which means that implementing PSR can possibly be alternative to more costly multi-antenna APs in those scenarios.



==> bibelo.tex <==
%% Eloise's references

@article{afaqui2016ieee,
  title={{IEEE 802.11 ax: Challenges and requirements for future high efficiency WiFi}},
  author={Afaqui, M Shahwaiz and Garcia-Villegas, Eduard and Lopez-Aguilera, Elena},
  journal={IEEE Wireless Communications},
  volume={24},
  number={3},
  pages={130--137},
  year={2016},
  publisher={IEEE}
}

@misc{GarGerGal2018,
  title={{Massive {MIMO} Unlicensed: {A} New Approach to Dynamic Spectrum Access}},
   author={Garcia-Rodriguez, Adrian and others},
 Howpublished={IEEE Communications Magazine},
  year={2018},
  volume={56},
  number={6},
  pages={186-192}
}

% @misc{GarGerGal2018,
%   author={Garcia-Rodriguez, Adrian and others}
%   journal={IEEE Communications Magazine}, 
%   title={Massive {MIMO} Unlicensed: {A} New Approach to Dynamic Spectrum Access}, 
%   year={2018},
%   volume={56},
%   number={6},
%   pages={186-192},}

 @ARTICLE{KhoLevAky2020,
  author={E. {Khorov} and I. {Levitsky} and I. F. {Akyildiz}},
  journal={IEEE Access}, 
  title={Current Status and Directions of {IEEE} 802.11be, the Future {Wi-Fi} 7}, 
  year={2020},
  volume={8},
  number={},
  pages={88664-88688},}
  
@misc{psrContribution,
  title={{Performance of parameterized spatial reuse (PSR) with coordinated beamforming/null steering for 802.11be}},
   author={Garcia-Rodriguez, Adrian and others},
  Howpublished={IEEE 802.11-20/0091r2},
  volume={},
  number={},
  pages={},
  year={Jan. 2020},
  publisher={}
}



@misc{qu2019survey,
  title={{Survey and performance evaluation of the upcoming next generation WLANs standard - IEEE 802.11ax}},
  author={Qu, Qiao and others},
  Howpublished={Mobile Networks and Applications},
  volume={24},
  number={5},
  pages={1461--1474},
  year={2019},
  publisher={Springer}
}

@misc{lopez2019ieee,
  title={{IEEE 802.11be Extremely High Throughput: The Next Generation of Wi-Fi Technology Beyond 802.11ax}},
  author={L{\'o}pez-P{\'e}rez, David and others},
  Howpublished={IEEE Communications Magazine},
  volume={57},
  number={9},
  pages={113--119},
  year={2019},
  publisher={IEEE}
}

@article{ieee,
  title={{P802.11ax/D6.0 - IEEE Draft Standard for Information
Technology - Specific Requirements
Part 11: Wireless LAN Medium Access Control (MAC) and
Physical Layer (PHY) Specifications}},
  author={},
  journal={IEEE 802.11},
  volume={},
  number={},
  pages={},
  year={November 2019},
  publisher={}
}

@article{broadband,
  title={{Evolved Universal Terrestrial Radio Access (E-UTRA); Further advancements for E-UTRA physical layer aspects}},
  author={},
  journal={3GPP TR 36.814},
  volume={},
  number={},
  pages={},
  year={March 2017},
  publisher={}
}

@article{lowlatency,
  title={{Study on physical layer enhancements for NR ultra-reliable and low latency case (URLLC)}},
  author={},
  journal={3GPP TR 38.824},
  volume={},
  number={},
  pages={},
  year={March 2019},
  publisher={}
}

@article{3gpp,
  title={{Study on channel model for frequencies from 0.5 to  100 GHz}},
  author={},
  journal={3GPP TR 38.901},
  volume={},
  number={},
  pages={},
  year={June 2018},
  publisher={}
}

@book{perahia2013next,
  title={{Next generation wireless LANs: 802.11n and 802.11ac}},
  author={Perahia, Eldad and Stacey, Robert},
  year={2013},
  publisher={Cambridge university press}
}

@online{cisco_2020, 
title={{Cisco Annual Internet Report (2018–2023) White Paper}}, url={https://bit.ly/3cgTKxa}, 
journal={Cisco}, 
publisher={Cisco}, 
year={2020}, 
month={Mar}}

@article{khorov2018tutorial,
  title={{A tutorial on IEEE 802.11ax high efficiency WLANs}},
  author={Khorov, Evgeny and Kiryanov, Anton and Lyakhov, Andrey and Bianchi, Giuseppe},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={21},
  number={1},
  pages={197--216},
  year={2018},
  publisher={IEEE}
}

@misc{deng2017ieee,
  title={{IEEE 802.11ax: highly efficient WLANs for intelligent information infrastructure}},
  author={Deng, Der-Jiunn and others},
  Howpublished ={IEEE Communications Magazine},
  volume={55},
  number={12},
  pages={52--59},
  year={2017},
  publisher={IEEE}
}

@article{wilhelmi2019spatial,
  title={{Spatial Reuse in IEEE 802.11ax WLANs}},
  author={Wilhelmi, Francesc and {S. Barrachina-Mu{\~n}oz} and Cano, Cristina and Selinis, Ioannis and Bellalta, Boris},
  journal={arXiv preprint arXiv:1907.04141},
  year={2019}
}

@inproceedings{shen2018research,
  title={{Research and Performance Evaluation of Spatial Reuse Technology for Next Generation WLAN}},
  author={Shen, Zhao and others},
  booktitle={International Wireless Internet Conference},
  pages={41--51},
  year={2018},
  organization={Springer}
}

@inproceedings{wilhelmi2019performance,
  title={{On the Performance of the Spatial Reuse Operation in IEEE 802.11ax WLANs}},
  author={Wilhelmi, Francesc and {S. Barrachina-Mu{\~n}oz} and Bellalta, Boris},
  booktitle={2019 IEEE Conference on Standards for Communications and Networking},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@article{valkanis2019ieee,
  title={{IEEE 802.11ax spatial reuse improvement: An interference-based channel-access algorithm}},
  author={Valkanis, Anastasios and Iossifides, Athanasios and Chatzimisios, Periklis and Angelopoulos, Marios and Katos, Vasilis},
  journal={IEEE Vehicular Technology Magazine},
  volume={14},
  number={2},
  pages={78--84},
  year={2019},
  publisher={IEEE}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@book{gast2005802,
  title={802.11 wireless networks: the definitive guide},
  author={Gast, Matthew},
  year={2005},
  publisher={O'Reilly Media, Inc.}
}



@ARTICLE{4804716,
author={L. J. Greenstein and S. S. Ghassemzadeh and V. Erceg and D. G. Michelson},
journal=IEEE_J_VT,
title={Ricean {K}-Factors in Narrow-Band Fixed Wireless Channels: {T}heory, Experiments, and Statistical Models},
year={2009},
volume={58},
number={8},
pages={4000-4012},
keywords={Rician channels;statistical analysis;Ricean K-factor;fading channel;frequency 1.9 GHz;narrow-band fixed wireless channel;statistical model;suburban macrocell;$K$-factors;Fading;Ricean distribution;fixed wireless channels;multipoint communication},
doi={10.1109/TVT.2009.2018549},
ISSN={0018-9545},
month={Oct.},}



%% Previous references

@book{80211,
author = "IEEE",
title = {{Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) Specifications}},
publisher = "IEEE Std. 802.11",
year = 1999}

@book{ASTM03,
author = "ASTM",
title = "Standard Specification for Telecommunications and Information Exchange Between Roadside
and Vehicle Systems  5 GHz Band Dedicated Short Range Communications (DSRC) Medium Access
Control (MAC) and Physical Layer (PHY) Specifications",
publisher = "ATSM Std. E2213-03",
year = 2003}

@article{Abel93,
    author = "Jonathan S. Abel",
    title = "A bound on Mean-Square-Estimate Error",
    journal = ieeetit,
    volume = 39,
    number = 5,
    pages = "1675--1680",
    month = sep,
    year = 1993}

@article{AbouFaycal01,
    author = "Ibrahim C. Abou-Faycal and Mitchell D. Trott and Shlomo Shamai",
    title = "The Capacity of Discrete-Time Memoryless {R}ayleigh-Fading Channels",
    journal = ieeetit,
    volume = 47,
    number = 4,
    pages = "1290--1301",
    month = may,
    year = 2001}

@book{AbramStegun,
    editor = "Milton Abramowitz and Irene A. Stegun",
    title = "Handbook of Mathematical Functions, 5th printing",
    publisher = dover,
    address = "New York",
    year = 1968}

@inproceedings{Agarwal06,
    author = "Manish Agarwal and Michael L. Honig and Baris Ata",
    title = "Adaptive Allocation of Pilot and Data Power for Time-Selective Fading Channels with Feedback",
    year = "submitted to ISIT 2006"}

@article{Agrell2002,
    author = "Erik Agrell and Thomas Eriksson and Alexander Vardy
        and Kenneth Zeger",
    title = "Closest Point Search in Lattices",
    journal = ieeetit,
    volume = 48,
    number = 8,
    pages = "2201--2214",
    month = aug,
    year = 2002}

@inproceedings{AiryVTC06,
    author = "Manish Airy and S. Bhadra and  {R. W. Heath Jr.}  and  S. Shakkottai",
    title = "Transmit Precoding for the Multiple Antenna Broadcast Channel",
    booktitle = "Proc. of the IEEE Veh. Tech. Conference",
    address = "Melbourne, Australia",
    volume = 3,
    pages = "1396-1400",
    month = may,
    year = 2006}


@ARTICLE{KalBor2017,
author    = {Elham Kalantari and
               Irem Bor{-}Yaliniz and
               Abbas Yonga{\c{c}}oglu and
               Halim Yanikomeroglu},
  title     = {User Association and Bandwidth Allocation for Terrestrial and Aerial
               Base Stations with Backhaul Considerations},
journal = {\emph{Available as} arXiv:1709.07356, \emph{Sept. 2017}.}
}

@ARTICLE{NewAmerica2015,
author={{New America}}, 
title={Drones and aerial observation: New technologies for property rights, human rights, and global development -- {A} primer},
year={2015}, 
month={July},
}

@INPROCEEDINGS{7536859,
author={V. V. Chetlur Ravi and H. S. Dhillon},
booktitle={Proc. IEEE SPAWC},
title={Downlink coverage probability in a finite network of unmanned aerial vehicle {(UAV)} base stations},
year={2016},
volume={},
number={},
pages={1-5},
month={July},
}

@ARTICLE{1043857,
author={H. Fattah and C. Leung},
journal=IEEE_M_WC,
title={An overview of scheduling algorithms in wireless multimedia networks},
year={2002},
volume={9},
number={5},
pages={76-83},
month={Oct.},
}

@ARTICLE{6415397,
author={H. Yin and D. Gesbert and M. Filippou and Y. Liu},
journal=ieeejsac,
title={A Coordinated Approach to Channel Estimation in Large-Scale Multiple-Antenna Systems},
year={2013},
volume={31},
number={2},
pages={264-273},
month={Feb.},
}

@book{MarLarYanBook2016,
editor = {Thomas L. Marzetta and Erik G. Larsson and Hong Yang and Hien Quoc Ngo},
title = {Fundamentals of Massive {MIMO}},
publisher = cup,
year = 2016}

@ARTICLE{MozSaaBen2017,
author={M. Mozaffari and W. Saad and M. Bennis and M. Debbah}, 
title={Communications and Control for Wireless Drone-Based Antenna Array},
journal = {\emph{Available as} arXiv:1712.10291, \emph{Dec. 2017}.}
}
